On the (ir)rationality of Kontsevich weights

We compute the weight of a Kontsevich graph in deformation quantization. Up to rationals, the result is Zeta(3)^2/Pi^6.

==> figthegraph.tex <==
\psset{unit=.5cm}
\psset{arrowscale=1}
\begin{pspicture}(0,-1)(8,4)  
  \cnode*(1,3){3pt}{a1}
  \cnode*(2,3){3pt}{a2}
  \cnode*(3,3){3pt}{a3}
  \cnode*(4,3){3pt}{a4}

  \cnode*(5,3){3pt}{z}  
  \cnode*(6,3){3pt}{w}
  \cnode*(7,3){3pt}{b}

  \cnode*(3,0){3pt}{l}  
  \cnode*(5,0){3pt}{r}
  
  \psline{-}(0,0)(8,0)
  \psset{arrows=->}
  \ncline{a1}{a2}
  \ncline{a2}{a3}
  \ncline{a3}{a4}
  \ncline{a4}{z}
  \ncline{z}{w}
  \ncline{b}{w}
  
  \ncline{a1}{l}
  \ncline{a2}{l}
  \ncline{a3}{l}
  \ncline{a4}{l}
  \ncline{w}{l}
  \ncline{z}{r}
  \ncline{w}{r}
  \ncline{b}{r}


  \uput{1ex}[-90](l){$U$}
  \uput{1ex}[-90](r){$V$}  

  \uput{1ex}[90](a1){$a_1$}
  \uput{1ex}[90](a2){$a_2$}  
  \uput{1ex}[90](a3){$a_3$}
  \uput{1ex}[90](a4){$a_4$}  
  \uput{1ex}[90](z){$z$}
  \uput{1ex}[90](w){$w$}  
  \uput{1ex}[90](b){$b$}
\end{pspicture}
